Meta-learning via Language Model In-context Tuning

The goal of meta-learning is to learn to adapt to a new task with only a few labeled examples. To tackle this problem in NLP, we propose $\textit{in-context tuning}$, which recasts adaptation and prediction as a simple sequence prediction problem: to form the input sequence, we concatenate the task instruction, the labeled examples, and the target input to predict; to meta-train the model to learn from in-context examples, we fine-tune a pre-trained language model (LM) to predict the target label from the input sequences on a collection of tasks. We benchmark our method on two collections of text classification tasks: LAMA and BinaryClfs. Compared to first-order MAML which adapts the model with gradient descent, our method better leverages the inductive bias of LMs to perform pattern matching, and outperforms MAML by an absolute $6\%$ AUC ROC score on BinaryClfs, with increasing advantage w.r.t. model size. Compared to non-fine-tuned in-context learning (i.e. prompting a raw LM), in-context tuning directly learns to learn from in-context examples. On BinaryClfs, in-context tuning improves the average AUC-ROC score by an absolute $10\%$, and reduces the variance with respect to example ordering by 6x and example choices by 2x.

==> arr-january-rebuttal.tex <==
% \section*{Summary of contribution}

% In this work, we propose a few-shot meta-learning method called in-context tuning (ICT), where few-shot task adaptation is performed by in-context learning. ICT recasts few-shot task adaptation and task-specific prediction as a simple sequence prediction problem, where the task instruction, few-shot examples, and the query example are concatenated to form the input sequence. To meta-train the ICT model, we fine-tune a pre-trained language model (LM) to learn the in-context sequence prediction problem on a collection of tasks. Compared to optimization-based meta-learning methods (e.g., MAML) which use gradient updates for task adaptation, model weights are frozen during task adaptation in ICT. 

% Extensive experiments on two meta-datasets LAMA and BinaryClfs show that our proposed ICT method outperforms in accuracy both in-context learning with off-the-shelf pre-trained LMs and classical few-shot meta-learning methods such as MAML. Furthermore, sensitivity analysis shows that ICT effectively alleviates the well-known oversensitivity issue of prompting off-the-shelf pre-trained LMs, significantly reducing the performance variance with respect to few-shot example selection, few-shot example ordering, and instruction wording.


\section*{Response to reviewers}

We thank the reviewers for their valuable feedback. We are glad to see that all reviewers agree on the practical importance and impact of the proposed in-context tuning approach, in terms of both improved performance accuracy and reduced sensitivity. We are also glad to see that all reviewers agree that the experiments are thorough and indicate the advantages of the proposed approach. 

We addressed reviewers' feedback in this version of the paper. We added reference to soft prompt work in the related work section, and explained the relation between in-context tuning and soft prompt tuning in the author response (AC 42WN's W1). We improved paper writing to clarify questions from reviewers regarding the MAML introduction (Reviewer HRgK's Q1), the variance decomposition formula (Reviewer HRgK's Q2), and the LAMA dataset (Reviewer fqjM's Q1). 

Note that all line numbers in the following responses refer to the revised version of the paper. 

\subsection*{Response to Area Chair 42WN}

W1: The paper doesn't mention any work on soft prompts. 

A: We view in-context tuning as orthogonal to soft prompt tuning. While soft prompts are updated via gradient descent on few-shot examples during task adaptation, both model weights and prompt weights are frozen during task adaptation in in-context learning. Soft prompt tuning is more similar to our baseline InsT + FT, where weights (either prompt weights or model weights) are updated with gradient descent during task adaptation. 

Our in-context tuning approach also enjoys the space efficiency of soft prompt tuning, as only one in-context tuned model needs to be tuned and stored for multiple downstream tasks. 

We have added reference to soft prompt tuning \citet{li-liang-2021-prefix, lester2021power, qin-eisner-2021-learning} to the Related Work section. 

\subsection*{Response to Reviewer HRgK}

Q1: The MAML introduction only mentions $S_T$ but not $D_T$. Does MAML use less data?

A: In-context tuning and all few-shot learning baselines (including MAML) always use the same shot number $K$ for fair comparison. $D_T$ refers to all labeled examples available for task $T$ (line 131-140). The size of $D_T$ can be much larger than the shot number $K$. To simulate $K$-shot learning during meta-training and meta-testing, we randomly sample a size-$K$ subset $S_T \subseteq D_T$ as few-shot examples available. We have modified the MAML section to clarify that $S_T$ is sampled from $ D_{T}$ (line 200, 207). \\

\noindent Q2: The three sources of variances are not independent (e.g., order variance depends on the choice). Therefore, the sensitivity decomposition formula is incorrect (line 445-447).

A: We define example choice $S_T$ as a random \emph{unordered} set of few-shot training examples with size $K$, and example ordering $\sigma$ as a random permutation of $K$ examples (line 436-438). Because $S_T$ is \emph{unordered}, order variance does not depend on the choice. The independence between the three sources of variance warrants the variance decomposition. We added an explanation of the independence between order variance and choice variance in line 443-444. \\

\noindent W1: The paper doesn't mention any work on soft prompts. 

A: Please see our response to AC 42WN’s W1. 

\subsection*{Response to Reviewer U3Y3}

W1: The novelty of this work is limited. 

A: While our work is inspired by the idea of instruction tuning \cite{wei2021finetuned}, the empirical results are strong and produce new takeaways/insights: 1) as pointed out by the meta review, few-shot learning is a more practical and impactful setting than zero-shot learning, 2) in-context tuning is a new way to do meta-learning and can be potentially extended to other applications, 3) in-context tuning can effectively reduce performance variance from in-context examples. \\

\noindent C1: The model considered in this paper is still relatively speaking small.

A: As we pointed out in Section~\ref{sec:future}, scaling up is an important future direction (line 581-598). For the models we experimented in this work, results in Table~\ref{tab:ict-vs-baselines} show that the performance improvement of in-context tuning over in-context learning with off-the-shelf pre-trained LMs increases as model size scales up (LAMA: +6.7 points for BERT-Base, +7.7 points for BERT-Large, \textbf{+8.5} points for DeBERTa-xlarge; BinaryClfs: +9.6 points for GPT2-Medium, \textbf{+11.5} points for GPT2-Large). 

\subsection*{Response to Reviewer kRRq}

W1: The improvements of in-context tuning over InsT + FT is marginal (Table~\ref{tab:ict-vs-baselines}).

A: While the InsT + FT baseline is competitive with in-context tuning, we observe that the advantage of in-context tuning over InsT + FT increases as model size scales up (-0.4 point for BERT-Base, +0.4 point for BERT-Large, \textbf{+1.8} points for DeBERTa-xlarge). We elaborate the observations in line 390-400. \\

\noindent W2: Two datasets may not be enough to support the claim in line 114.

A: Both LAMA and BinaryClfs are meta-datasets, i.e., collections of datasets. The LAMA meta-dataset we use contains 29 distinct tasks, while BinaryClfs contains 204 distinct tasks (Section~\ref{sec:dataset-and-metrics}). Hence, the two meta-datasets are highly rich in dataset diversity, which adds validity to our claim. \\

\noindent W3: Evaluation should include more recent methods in meta-learning.

A: We choose MAML as our meta-learning baseline because it is one of the most widely used meta-learning algorithms in NLP and is representative of the broader family of optimization-based meta-learning methods (Section~\ref{sec:gradient-based-adapt}). 

\subsection*{Response to Reviewer fqjM}

W1: The novelty of this work is limited. 

A: Please see our response to U3Y3’s W1. \\

\noindent W2: The paper does not compare with PET.

A: As a semi-supervised approach, PET assumes access to large unlabeled datasets, which are sometimes unavailable in practical settings. Our work chooses not to have this assumption. \\

\noindent Q1: Why are the reported precision scores on LAMA much lower than 50\%?

A: We use the same evaluation protocol as in \citet{petroni-etal-2019-language}: the object entity is predicted from a pre-defined vocabulary set of 21k words (line 278-281). Hence, each LAMA relation is a 21k-way classification task as opposed to a binary classification task, which is why precision scores are much lower than than 50\%. We modified the introduction of LAMA to explicitly mention that each LAMA relation is a 21k-way classification task (line 281). \\

\noindent Q2: The ICT framework supports multi-class classification tasks, thus allowing the comparison with existing works. Why do the authors modify the LAMA and BinaryClfs datasets?

A: It's true that multi-class classification is not an issue, and we modify the two datasets not to change multi-class classification to binary classification. 

We modify LAMA because initial experiments reveal that LMs take significant advantage of “majority label bias” \cite{zhao2021calibrate}, where they assign higher probability to object entities that have appeared in the in-context examples, thus significantly inflating the accuracy (line 262-270). While we agree that modifying the dataset will make it harder to compare the numbers reported in our work with other work, we believe it's important to reflect the improvement due to few-shot learning rather than this simple heuristic to copy answers. Hence, for all tasks we prune the LAMA dataset so that all object entities appear less than 2.5\% of times (line 266-272).

For BinaryClfs, we removed a few tasks where example inputs are too long to fit into the context window size of a GPT-2 model when in-context learning is used (line 298-302). As we mentioned in Section~\ref{sec:future}, one future direction is to scale up the number of few-shot examples, which can be accommodated with models with longer context size \cite{dai-etal-2019-transformer, wang2020linformer}.
